A Hierarchical Deep Convolutional Neural Network and Gated Recurrent Unit Framework for Structural Damage Detection

Structural damage detection has become an interdisciplinary area of interest for various engineering fields, while the available damage detection methods are being in the process of adapting machine learning concepts. Most machine learning based methods heavily depend on extracted ``hand-crafted" features that are manually selected in advance by domain experts and then, fixed. Recently, deep learning has demonstrated remarkable performance on traditional challenging tasks, such as image classification, object detection, etc., due to the powerful feature learning capabilities. This breakthrough has inspired researchers to explore deep learning techniques for structural damage detection problems. However, existing methods have considered either spatial relation (e.g., using convolutional neural network (CNN)) or temporal relation (e.g., using long short term memory network (LSTM)) only. In this work, we propose a novel Hierarchical CNN and Gated recurrent unit (GRU) framework to model both spatial and temporal relations, termed as HCG, for structural damage detection. Specifically, CNN is utilized to model the spatial relations and the short-term temporal dependencies among sensors, while the output features of CNN are fed into the GRU to learn the long-term temporal dependencies jointly. Extensive experiments on IASC-ASCE structural health monitoring benchmark and scale model of three-span continuous rigid frame bridge structure datasets have shown that our proposed HCG outperforms other existing methods for structural damage detection significantly.

==> abstract.tex <==

          

==> preliminary.tex <==
\section{Preliminaries}

\subsection{Convolution Neural Network}
CNN is an artificial neural network with deep learning ability, which is inspired by the visual structure model of cat proposed by Hubel et al in 1962. The classic LeNet~\cite{lecun1998gradient} et al were born in 1998. however, due to the limited computing power at that time, its advantages have not been explored. In recent years, convolution neural network has been widely used in search and retrieval, image understanding, speech recognition, mobile phone applications, map navigation, medical and pharmaceutical, UAV and driverless vehicles and other fields.
A plurality of sensors are installed on the structure, which form a vector matrix, as shown in figure 1. The features are extracted by one-dimensional convolution CNN, each layer of CNN contains several convolution cores of the same size. Each convolution kernel produces a new data order, which merges the data extracted by multiple convolution kernels as the input data of GRU.
\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.4]{cnn.png}
    \caption{1 dimensional CNN convolution neural network.}
    \label{fig:1 dimensional CNN convolution neural network}
\end{figure}
Because of too many weights, the effect of conventional neural network in dealing with large-scale data is not ideal, while CNN effectively solves the problem that large-scale data network can not learn through weight sharing and local connection. CNN reduces the parameters and improves the efficiency through local connection, weight sharing and aggregation layer (Pooling). CNN can retain and extract features from topological data, which is why it is suitable for dealing with pictures and audio.

\subsection{Recurrent Neural Networks}
Cyclic neural network (Recurrent Neural Networks,RNN) is a general name of neural network structure which is specially used to deal with sequence data. As shown in figure 2, for the basic RNN structure, the network feeds back the state of the neuron at the previous moment and acts as an input to the neuron to capture the historical information of the sequence. A feed forward neural network with a width of sequence length is obtained by expanding RNN according to time. When the back propagation algorithm is used to update the RNN parameters, the problem of gradient explosion and disappearance will occur. The problem of long-term dependence on (Long Term Dependency) without long-term memory ability leads to the serious limitation of the application of RNN.
\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.3]{rnn.png}
    \caption{Basic RNN expansion diagram.}
    \label{fig:Basic RNN expansion diagram.}
\end{figure}

LSTM network is an improved time cyclic neural network. The cyclic structure of  LSTM consists of three control gates: forgetting gate (forget gate), external input gate (external input gate) and output (output gate). Thus, the problem of "gradient disappearance" in RNN model training is solved, and it can learn the long-term and short-term dependence information of time series, and can be applied in many scenarios. Where GRU is an important variant of LSTM proposed by Cho, as shown in figure 3. GRU combines the amnesia gate with the input gate into a single update gate, mixing the cellular state and the hidden state, and the final model is simpler than the standard LSTM model.


The basic idea of GRU is that only the forgotten state part is updated with candidate output. Because GRU has only two control gates, reset gate and update gate, the calculation speed of GRU is much faster than that of LSTM. The main function of update gate $r^t$, is to control which information is retained in the current input, and the main function of reset gate $h^t-1$ is to control the influence of the output of the previous moment on the current input $r^t$.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.2]{GRU.png}
    \caption{GRU Element Model.}
    \label{fig:GRU Element Model.}
\end{figure}



